Learning materials spectra across modalities and scales with structure-conditioned neural fields

Spectroscopic observables encode rich information about material behavior across diverse, often high-dimensional domains of energy, momentum, and other experimental coordinates, providing critical insights into the physical properties underlying material functionalities and applications. However, learning these responses directly from atomic structures remains challenging due to the complexity of both structural configurations and spectroscopic observation spaces. Here, we develop a structure-conditioned neural-field framework that learns continuous spectroscopic response functions by coupling an equivariant structural encoder with a coordinate-conditioned network. The framework accurately predicts spectroscopic observables across diverse observation domains, ranging from one-dimensional densities of states to multidimensional scattering functions. We show that fine-tuning with limited spectral supervision captures strain- and composition-dependent spectral changes, with validated transfer to alloy configurations containing hundreds of atoms and computational scalability demonstrated for configurations exceeding $10^4$ atoms. Our work establishes a versatile and computationally scalable approach to learning structure-spectroscopy relationships, providing a foundation for spectroscopic analysis and future materials characterization, inverse problems, and experimental design.

==> captions/figure1.tex <==
\caption[Figure 1]{%
\textbf{Structure-conditioned spectral fields across observation domains.}
\textbf{a,} SpecSCoNe illustrated for powder INS. An equivariant encoder maps a crystal structure \(X\) to a material representation \(\mathbf z_X\), which conditions a coordinate network \(f_\theta\) to predict intensity at momentum-transfer magnitude \(Q=|\mathbf Q|\) and energy transfer \(E\). The surface depicts a reference powder spectrum, with height and colour encoding intensity; the highlighted point marks the queried location.
\textbf{b,} Reference spectra across one-, two- and four-dimensional observation domains: PhDOS and eDOS profiles and a powder-INS map for MgO, and single-crystal INS for BaF$_2$. Each single-crystal stack contains \(Q_x\)--\(Q_y\) sections at different \(Q_z\) values and a fixed energy.
}


==> captions/figure2.tex <==
\caption[Figure 2]{%
\textbf{Spectroscopic fidelity across materials and observables.}
\textbf{a,} Predicted versus reference integrated intensity, energy centroid and energy-distribution width, and the distribution of Wasserstein-1 distances \(W_1\), for 1,001 powder-INS test materials. Quantities are calculated from \(Q\)-integrated energy profiles, with area normalization for \(W_1\). Dashed lines indicate equality.
\textbf{b,} Top, reference energy centroid \(\mu_E\) versus compositional lightness \(L_{\min}\) for test materials, coloured by N-L2. Contours show training-set density; the pale vertical band labelled H identifies hydrogen-containing materials. Bottom, median N-L2 in groups E1--E4 defined by training-set reference-centroid quartiles. Open and filled markers denote validation and test medians, respectively; whiskers indicate the interquartile range.
\textbf{c,} Validation examples from task-specific N-L2 quartiles D1--D4, ordered by increasing error. Left, the powder-INS error distribution and selected examples near the 5th, 35th, 65th and 90th percentiles. Constant-\(Q\) profiles correspond to \(Q=6.55\)~\AA$^{-1}$ (dashed lines on the maps). Right, PhDOS, NWDOS, 1D INS and eDOS predictions compared with Gaussian-smoothed references. Dark curves denote references; prediction colours identify D1--D4. Reference and prediction share an intensity scale within each powder-map pair and profile comparison. Powder maps and constant-\(Q\) profiles display 0--100~meV; errors are evaluated over the complete reference grids. For the one-dimensional profiles, energy is plotted horizontally, relative to the Fermi energy \(E_F\) for eDOS; numerical tick labels are omitted. Full-range powder and one-dimensional comparisons with labelled axes are provided in Supplementary Figs.~\ref{fig:si-powder-atlas} and~\ref{fig:si-1d-atlas}, respectively.
}


==> captions/figure3.tex <==
\caption[Figure 3]{%
\textbf{Learning spectroscopic responses across structural variations and scales.}
\textbf{a,} WSe$_2$ under biaxial strain. Left, DFT-derived spectra at $-2\%$, 0 and $+2\%$. Right, the withheld $+0.5\%$ response, \(\Delta S=S_{+0.5\%}-S_0\), from DFT, the globally trained model (Global) and the strain-adapted model (Adapted). Each difference uses the corresponding unstrained spectrum; red and blue indicate intensity gain and loss.
\textbf{b,} Composition adaptation in 12-atom \(\mathrm{Mo}_{1-x}\mathrm{W}_x\mathrm{S}_{2(1-y)}\mathrm{Se}_{2y}\) configurations, where \(x\) and \(y\) denote W and Se fractions. A separate model is adapted on 15 compositions and evaluated on 30 withheld compositions. Reference, global and composition-adapted spectra are shown for the highlighted withheld composition, \((x,y)=(0.75,0.75)\).
\textbf{c,} PCA projection of the composition-adapted material representations. Filled and open points denote training and withheld compositions; lines connect adjacent points in the composition grid. Surrounding maps show predictions at selected boundary compositions.
\textbf{d,} Reference and predicted powder maps and \(Q\)-integrated energy profiles for an independently randomized and relaxed \(10\times10\), 300-atom configuration at the withheld composition \((x,y)=(0.25,0.625)\), using the composition-adapted model without further training.
\textbf{e,} Prediction for a \(62\times62\), 11,532-atom alloy configuration using the same model on a single GPU, shown alongside the atomic structure and a magnified region. No reference spectrum was generated; this example assesses computational capacity rather than spectral fidelity.
Reference spectra were calculated from DFT forces in \textbf{a} and MACE forces in \textbf{b,d}. Maps display 0--60~meV, with shared colour scales within each comparison. Additional results are provided in Supplementary Note~\ref{note:f3}.
}


==> captions/figure4.tex <==
\caption[Figure 4]{%
\textbf{Spectroscopy-informed material representations and coordinate-based spectral analysis.}
\textbf{a,} Crystal structures (top), reference powder-INS maps (middle) and eDOS profiles (bottom) for BaCl$_2$ (A), PrIn$_2$Cl$_5$ (B) and LiI (C). INS energies are in meV; eDOS energies are relative to \(E_F\), in eV.
\textbf{b,} Ranks of B and C among the 718 other validation materials, ordered by representation-space cosine distance from A, at initialization and after INS, eDOS or joint supervision.
\textbf{c,} Neighborhood enrichment across 649 test materials, defined as the fractional reduction in mean reference-spectral distance relative to random selection. For each model and query, the same five nearest neighbors in representation space are evaluated using reference INS and eDOS spectra. Error bars indicate 95\% confidence intervals obtained by bootstrapping test queries.
\textbf{d,} Local \(Q\)-integrated energy profile for the withheld alloy composition \((x,y)=(0.25,0.50)\), estimated from 90 coordinate queries within the indicated momentum--energy window. The blue marker denotes the energy centroid. The high-energy intensity fraction is the integrated intensity above 30~meV (orange shading) divided by that over the selected window.
\textbf{e,} Reference and predicted MoSe$_2$ profiles at $-1.5\%$, 0 and $+1.5\%$ strain (top), with dashed markers indicating tracked ridge positions. Predicted versus DFT-derived ridge-shift coefficients \(\alpha\) for four TMDs at withheld \(\pm0.5\%\) strain (bottom), expressed as energy shifts per percentage point of biaxial strain.
\textbf{f,} Sampling-budget dependence of errors relative to estimates from densely sampled model spectra: energy-centroid mean absolute error (MAE) across 30 withheld compositions (top) and ridge-shift coefficient MAE across four compounds, using stored spectra at 0 and \(\pm1.5\%\) strain (bottom). Shading in the top panel indicates 95\% confidence intervals obtained by bootstrapping compositions. Sampling fractions are relative to the corresponding full spectral grids.
\textbf{g,} Recorded computation times for complete powder-INS spectra for relaxed WSe$_2$ (top) and 12--300-atom alloys (bottom). The MLFF-based workflows use EquiformerV3 and MACE, respectively. DFT timing includes summed force-job wall times and spectral post-processing. Alloy curves and shading show medians and ranges across two configurations per size; the dashed curve shows the OCLIMAX contribution under the fixed protocol including coherent scattering (Methods; Supplementary Note~\ref{note:f4}).
}

